Scalable UTXO Smart Contracts via Fine-Grained Distributed State

UTXO-based smart contract platforms face an efficiency bottleneck, in that any transaction sent to a contract must specify the entire updated contract state. This requirement becomes particularly burdensome when the contract state contains dynamic data structures, as needed in many use cases to track interactions between users and the contract. The problem is twofold: on the one hand, a large state in transactions implies a large transaction fee; on the other hand, a large centralized state is detrimental to the parallelization of transactions - a feature that is often cited as a key advantage of UTXO-based blockchains over account-based ones. We propose a technique to efficiently execute smart contracts on an extended UTXO blockchain, which allows the contract state to be distributed across multiple UTXOs. In this way, transactions only need to specify the part of the state they need to access, reducing their size (and fees). We show how to exploit our model to parallelize the validation of transactions on multi-core CPUs. We implement our technique and provide an empirical validation of its effectiveness.

==> arxiv-experiments.tex <==
\subsection{Benchmarks}

\begin{comment}
pub use crowdfunding::*; % centralizzato e distribuito, parameter=number of donors
% quanto migliora la parallelizzazione wrt validazione parallela 
pub use two\_var::*; % due variabili X e Y, distribuito, random access ops
pub use rules::*; % HURF dummy contract: any one can deposit, owner can withdraw; no random ops
pub use etherdoc::*; % HURF notarization: register, claim, own; deadlines, spoof protection, no radom ops, parameter=numero di istanze del contratto, ogni contratto ha una singola register,...
pub use map::*; % HURF map: increment(map[x]++), parameter=conflict% for x, random ops 
% vedere quanto pesano i conflitti

pub use multisig::*; % HURF, authorize/deposit/transfer; parameter=numer of users, at least half needed to transfer, random ops
\end{comment}

The common goal of all our experiments is to measure the speedup obtained by distributing the contract state and by parallelizing the validation of transactions over multiple threads.
To this purpose, we consider a benchmark of contracts with different features, which we describe below.

\paragraph{Crowdfund}

The first use case is the crowdfund contract of~\Cref{sec:overview}.
The interest in this contract is that it includes methods that simultaneously update maps and transfer tokens, but still in a way that we expect to lead to an efficient parallelization.
This is because donors operate on disjoint parts of the state, and that token transfers from the contract are always guaranteed to be successful, so reducing conflicts.
%
The experiment compares the centralized implementation of this contract (\ie, the one that keeps the whole donors map in the $\txf{datum}$ field, copying it each time a new donor is added) \wrt a distributed implementation that uses the technique of~\Cref{sec:compilation} to distribute the state across multiple outputs.


\paragraph{Map}

This use case involves a basic contract that stores a map (see~\Cref{fig:map}).
The contract has a single rule, which allows anyone to update the value of the map at any given key.
This allows us experiment with different rates of soft conflicts: we can perform a bunch of updates on completely distinct keys ($0\%$ soft conflicts), we can update the map always on the same key ($100\%$ soft conflicts), or fine-tune the conflict probability to any intermediate level.
%
In this way, we aim to measure how performance is affected by the presence of soft conflicts.


\iftoggle{arxiv}{%
\begin{figure}
\lstinputlisting[language=rulecode,morekeywords={ConflictMap,inc}]{hurf/map.hurf}
\caption{The map contract in \rulelang.}
\label{fig:map}
\end{figure}
}
{}

\paragraph{Multisig wallet}

This use case implements a multisig wallet involving $N$ privileged users approved by the owner, where token transfers must be authorized by $K = N/2$ of them.
The contract (see~\Cref{fig:multisig}) has three rules.
The first rule allows the contract owner to add authorized users to the wallet.
%
The second rule allows anyone to deposit tokens within the wallet, without requiring any authorization.
%
The third rule allows to withdraw tokens from the contract: this is possible only when $K$ authorized users approve the withdrawal by signing the corresponding transaction.
%
The goal of this experiment is to measure the the impact of signatures, one of the most computationally expensive primitives of the blockchain.

\iftoggle{arxiv}{%
\begin{figure}
\lstinputlisting[language=rulecode,morekeywords={MultiSig_N,authorize,deposit,withdraw}]{hurf/multisig.hurf}
\caption{The Multisig wallet contract in \rulelang.}
\label{fig:multisig}
\end{figure}
}
{}

\paragraph{Registry}

This use case implements a registry contract, which allows users to register the hash of a document on the blockchain, and later to claim its ownership (\Cref{fig:registry}).
Users start by calling a rule to record in a map the \emph{hash of the hash} of their document, and a current timestamp.
This is needed to prevent frontrunning attacks where an adversary ``steals'' the actual document hash, and registers it before the legit user.
After that, the user calls another rule to reveal the actual hash, and store it in another map.
This rule allows the legit user (\ie, the first one to register the double hash) to overwrite any adversaries' claims. 
Finally, the user who has claimed a hash can permanently record its ownership.
The corresponding rule uses time constraints to ensure that the legit user can reveal the hash, as per the second rule.
The interest in this contract is in the combination of maps and hash functions; hashes are computed in the second and third rule to obtain the double hash.

\iftoggle{arxiv}{%
\begin{figure}
\lstinputlisting[language=rulecode,morekeywords={Registry,register,claim,own}]{hurf/registry.hurf}
\caption{The registry contract in \rulelang.}
\label{fig:registry}
\end{figure}
}

\subsection{Results}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Crowdfund
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iftoggle{arxiv}{\input{figures/tab-cf.tex}}{}

% \begin{figure*}
%     \centering
%     \begin{minipage}{0.495\textwidth}
%         \centering
%         \input{figures/fig-cf-time.tex}
%     \end{minipage}
%     \begin{minipage}{0.495\textwidth}
%         \centering
%         \input{figures/fig-cf-speedup.tex}
%     \end{minipage}
%     \vspace{-5pt}
%     \caption{Timings and speedup for the Crowdfund experiments.}
%     \label{fig:cf}
% \end{figure*}

\paragraph{Crowdfund}

We craft an experiment for the centralized and distributed versions of the contract, for each value of $N_{\it threads}$ (so encompassing both sequential and parallel validators), and for varying numbers of donors.
In each experiment, the input transaction sequence $\vec{T}$ has a prefix where all the donors make their donations, followed by a suffix where they claim a refund after the deadline.
%
\Cref{fig:cf} displays time needed to validate the sequence $\vec{T}$ in each experiment.

We first observe that, as the number of donors grows, the centralized version of contract becomes less and less efficient than the distributed one: this is because replicating the full state in each transaction output requires more time and memory. More precisely, each donation adds an entry in the donor map, making it larger, so the overall consumed memory is quadratic \wrt the number of donors. 
% Trying to increase the number of donors (\eg, up to \todo{con 64GB, 23K} 12K) resulted in memory exhaustion.
%
By contrast, the distributed contract scales linearly, so we managed to run it with a much larger number of users. 
\Cref{fig:cf} shows the amount of space required to store the blockchain in the centralized and distributed versions of the contract, for a varying number of users.
The figure confirms the expected quadratic behaviour (both in time and space) of the centralized version, and the linear behaviour of the distributed one.
% \Cref{tab:experiments:crowdfund} shows the results also for 50K users, but we also performed a single run with 500K users without running out of memory (in $28.5s$ with $1+7$ threads).

\zunnote{FIX ref}

From~\Cref{tab:cf} we also observe that the centralized contract executed by the parallel validator gets slower as the number of threads increases. This trend was expected, since the transactions in the centralized contract form a long chain where each one redeems the output of the previous one, preventing parallelization because of such a large number of soft conflicts. 
%
Increasing the number of threads only increases the contention between them.

The distributed contract instead benefits from the parallel validator, which becomes faster with more threads. Indeed, the experiment features many non-conflicting transactions since the state is distributed, allowing the parallel validator to exploit its threads. 
The percentage of (soft) conflicts, which only depends on the number of users,
% and not on the number of threads
drops steeply from $18.23\%$ in the experiments with 250 users, to $1.05\%$ in those with 50K users.
 % see results/cf-conflicts.csv
%
These conflicts are mostly due to the splitting and merging of map intervals (as per~\Cref{subsec:state-updates}) that occur during the $\ruleinline{donate}$ and $\ruleinline{refund}$ operations.
%
Effectively, these soft conflicts are caused by the implicit data dependencies as discussed in~\Cref{sec:parallelization}.

% \Cref{fig:cf} (right) shows the space speedup of the distributed contract over the centralized one, and the time speedup of the distributed contract with the parallel validator (with 1+7 threads) over the sequential/distributed contracts with the sequential validator. 
We observe that the time speedup of the distributed over the centralized contract grows linearly in the number of users.
% By comparing the two extremes, \ie the centralized version (with the sequential validator) and the distributed version (with the parallel validator), we observe a speedup of \todo{check} $13.04$ with $1 + 7$ threads. 
%
Instead, fixing the distributed contract, the time speedup of the parallel validator (with 1+7 threads) over the sequential one grows with the number of users, being only bounded by the number of available threads.
For instance, we have a $6.13$ speedup for $20K$ users and a $7.01$ speedup for $50K$ users.
This increase in the speedup is coherent with the reduced percentage of conflicts. 
% we observe a speedup of $2.81$ (with 8K users) and of $3.15$ (with $50K$ users). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Map
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Map}

% \begin{figure*}[t]
%     \centering
%     \begin{minipage}{0.495\textwidth}
%         \centering
%         \input{figures/fig-map-time.tex}
%     \end{minipage}
%     \begin{minipage}{0.495\textwidth}
%         \centering
%         \input{figures/fig-map-speedup.tex}
%     \end{minipage}
%     \vspace{-5pt}
%     \caption{Timings and speedup for the Map experiments.}
%     \label{fig:map}
% \end{figure*}

The goal here is to study the performance of the distributed Map contract under a varying conflicts probability.
%
Given a wanted probability $p$ of soft conflicts,
we construct a sequence of transactions~$\vec{T}$ with $50K$ \emph{random} calls of the rule $\ruleinline{inc}$, each time determining the actual parameter based on the toss of a biased coin. 
With probability $p$, we update $\ruleinline{m[0]}$;
%
with probability $1-p$, we update $\ruleinline{m[i]}$ where the index $i$ is incremented each time.
%
In this way, we repeatedly update the same map location $\ruleinline{m[0]}$ with probability $p$, ensuring a soft conflict each time.
%
By contrast, the other map updates access distinct locations $\ruleinline{m[i]}$, which is very unlikely to cause conflicts.
%
Indeed, in such cases a conflict happens only because of the implicit data dependencies discussed in~\Cref{sec:parallelization}, when 
two accesses $\ruleinline{m[i]}$ and $\ruleinline{m[j]}$ need to split the same interval.
%
Since the number of intervals increases after each $\ruleinline{m[i]}$ update, the probability of such conflicts quickly becomes very small, making the effective conflict probability be close to the wanted parameter $p$.

\Cref{fig:map} displays the results of our experiment with varying values of the conflict probability $p$ and with different validators.
%
We observe that the parallel validator is generally faster than the sequential one when using at least $2$ worker threads.
%
The sequential validator becomes faster when $p > 54\%$ (dotted vertical line in~\Cref{fig:map}), \ie when we have a very high conflict probability.
%
This corresponds to the highly unrealistic scenario where more than half of the transactions in the blockchain update the same map location. % of the same contract.
%
% Consequently, this scenario is far from the real-world.
%
When $p$ assumes more realistic values such as $p < 15\%$, we observe a $1.71$ speedup comparing the sequential validator to the parallel one ($1+3$ threads).

% idealmente, potremmo fare una figura come in Dickerson, dove:
% asse X: percentuale di conflitti (da stimare ex-post)
% asse Y: speedup (linee diverse per N_threads)
% E' vero che già l'esperimento Map fa questo, ma da quell'esperimento non si 
% riesce a inferire lo speedup per gli altri contratti
% Per ottenere una certa percentuale di conflitto, basterebbe avere un singolo utente
% che ogni tot donate degli altri fa la sua donate, mentre tutti gli altri fanno una
% sola donate a testa


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Multisig
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% bart: se mettiamo la figura, la tabella è ridondante
% \input{figures/tab-multisig.tex}

% \begin{figure*}
%     \centering
%     \begin{minipage}{0.495\textwidth}
%         \centering
%         \input{figures/fig-multisig-time.tex}
%     \end{minipage}
%     \begin{minipage}{0.495\textwidth}
%         \centering
%         \input{figures/fig-multisig-speedup.tex}
%     \end{minipage}
%     \vspace{-5pt}
%     \caption{Timings and speedup for the Multisig experiments.}
%     \label{fig:multisig}
% \end{figure*}


\paragraph{Multisig wallet}

We craft an experiment for the distributed version of the contract, varying the number $N$ of privileged users ($N = 2,4,6,10$) and the number of threads available to the validator.
In each experiment, the sequence of transactions $\vec{T}$ starts with the owner authorizing $N$ users, and then proceeds with $100K$ random operations. 
%
When the wallet holds no tokens, we perform a $\ruleinline{deposit}$ operation adding one token.
%
Otherwise, we flip an unbiased coin, and perform either 
a $\ruleinline{deposit}$ or a $\ruleinline{withdraw}$, both involving one token.
%
Each $\ruleinline{withdraw}$ operation is signed by $K=N/2$ users, so that it always succeeds. Consequently, to be executed it requires verifying $N/2$ signatures, plus an extra one to pay the transaction fees.
%
By contrast, $\ruleinline{authorize}$ operations only require verifying $2$ signatures (the owner's and the one for the fees), while $\ruleinline{deposit}$ operations require $2$ signatures (one for the deposited token and the one for the fees).
Overall, we measured \mbox{$\sim{1.5}\%$} of soft conflicts. This is not affected in any significant way by the number of users $N$, nor by the number of threads.

The results are displayed in~\Cref{fig:multisig}.
As expected, the average running time roughly scales with the average number of verified signatures. Assuming that the number of deposits is close to the number of withdraws, the number of verified signatures for $N$ participants can be estimated as $S(N) = 100K \cdot (0.5 \cdot 2 + 0.5 \cdot (N/2+1)) = 25K \cdot N + 150K$.
%
Observing the timings in~\Cref{fig:multisig} (left) we see that the time for each $N$ is roughly proportional to $S(N)$, confirming that the cost of signature verification is the main factor affecting performance.
%
\Cref{fig:multisig} (right) shows the speedups of the parallel validator over the sequential one for a varying number of threads. We observe that the speedup does not depend on the value of $N$ but only on the number of threads, confirming that contracts that make heavy use of signature verification can fully exploit parallel validation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Registry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Registry}

% \begin{figure*}
%     \centering
%     \begin{minipage}{0.495\textwidth}
%         \centering
%         \input{figures/fig-registry-time.tex}
%     \end{minipage}
%     \begin{minipage}{0.495\textwidth}
%         \centering
%         \input{figures/fig-registry-speedup.tex}
%     \end{minipage}
%     \vspace{-5pt}
%     \caption{Timings and speedup for the Registry experiments.}
%     \label{fig:registry}
% \end{figure*}

In each experiment, the input transaction sequence $\vec{T}$ starts with
% deploys the contract 
$N$ distinct users invoking $\ruleinline{register}$ on a document of their own.
%
The users then perform a $\ruleinline{claim}$ on their documents, wait for the deadlines to expire, and finally 
invoke $\ruleinline{own}$ to assert their ownership on the document they registered.
%
\Cref{fig:registry} displays the timings and speedup for the distributed version of the contract.
%
We observe that the parallel validator is significantly faster than the sequential one. 
Using $1+2$ threads, the speedup is always greater than $1$ even for a small number of users (\eg, it $1.47$ is for $N = 250$). 
Using $1+7$ threads, the speedup is always greater than $1$, and it tends asymptotically to the bound $7$ as the number of users grows.
%
This is due to a low number of soft conflicts (less than $2\%$).

==> figures/tab-multisig.tex <==
% cargo run -r -- --threads=0,1,2,3,4,5,6,7 --test=multisig2,multisig4,multisig6,multisig10 --runs=10

\begin{table}[h]
\centering
\csvreader[
    tabular = ccccc,
    table head = \toprule \textbf{Validator} & \textbf{Multisig2} & \textbf{Multisig4} & \textbf{Multisig6} & \textbf{Multsig10} \\\midrule,
    table foot = \bottomrule,
]{results/multisig.csv}
{
Validator=\validator,multisig2=\msigII,multisig4=\msigIV,multisig6=\msigVI,multisig10=\msigX}{%
% \tablenum[table-number-alignment = center,table-format = 5.0]{\numusers} 
\validator
& \msigII
& \msigIV
& \msigVI
& \msigX
}%
\caption{Timings for the Multisig experiments.}
\label{tab:multisig}
\end{table}
